Evidence for the volatile-rich composition of a 1.5-$R_\oplus$ planet

The population of planets smaller than approximately $1.7~R_\oplus$ is widely interpreted as consisting of rocky worlds, generally referred to as super-Earths. This picture is largely corroborated by radial-velocity (RV) mass measurements for close-in super-Earths but lacks constraints at lower insolations. Here we present the results of a detailed study of the Kepler-138 system using 13 Hubble and Spitzer transit observations of the warm-temperate $1.51\pm0.04~R_\oplus$ planet Kepler-138 d ($T_{\mathrm{eq, A_B=0.3}}$~350 K) combined with new Keck/HIRES RV measurements of its host star. We find evidence for a volatile-rich "water world" nature of Kepler-138 d, with a large fraction of its mass contained in a thick volatile layer. This finding is independently supported by transit timing variations, RV observations ($M_d=2.1_{-0.7}^{+0.6}~M_\oplus$), as well as the flat optical/IR transmission spectrum. Quantitatively, we infer a composition of $11_{-4}^{+3}$\% volatiles by mass or ~51% by volume, with a 2000 km deep water mantle and atmosphere on top of a core with an Earth-like silicates/iron ratio. Any hypothetical hydrogen layer consistent with the observations ($<0.003~M_\oplus$) would have swiftly been lost on a ~10 Myr timescale. The bulk composition of Kepler-138 d therefore resembles those of the icy moons rather than the terrestrial planets in the solar system. We conclude that not all super-Earth-sized planets are rocky worlds, but that volatile-rich water worlds exist in an overlapping size regime, especially at lower insolations. Finally, our photodynamical analysis also reveals that Kepler-138 c ($R_c=1.51 \pm 0.04~R_\oplus$, $M_c=2.3_{-0.5}^{+0.6}~M_\oplus$) is a slightly warmer twin of Kepler-138 d, i.e., another water world in the same system, and we infer the presence of Kepler-138 e, a likely non-transiting planet at the inner edge of the habitable zone.

==> commanddef.tex <==
\newcommand\ion[2]{#1$\,${\scshape{#2}}}  % ion, i.e., CII = \ion{C}{ii}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mt}[1]{\mathrm{#1}}
\newcommand{\Msun}{\ensuremath{\,M_{\odot}}}
\newcommand{\Mearth}{\ensuremath{\,M_{\oplus}}}
\newcommand{\Mmoon}{\ensuremath{\,M_{\mathrm{Moon}}}}
\newcommand{\Mjup}{\ensuremath{\,M_{\mathrm{Jup}}}}
\newcommand{\Rjup}{\ensuremath{\,R_{\mathrm{Jup}}}}
\newcommand{\mum}{\ensuremath{\,\mu}m}
\newcommand{\arcmin}{\ensuremath{^{\prime}}}
\newcommand{\arcsec}{\ensuremath{^{\prime\prime}}}
\newcommand{\farcmin}{\mbox{\ensuremath{.\mkern-4mu^\prime}}}%  % fractional arcminute symbol: 0.'0
\newcommand{\farcsec}{\mbox{\ensuremath{\,.\!\!^{\prime\prime}}}}%  % fractional arcsecond symbol: 0.''0
\newcommand{\water}{H$_{2}$O}

